A Two-Stage Approach towards Generalization in Knowledge Base Question Answering

Most existing approaches for Knowledge Base Question Answering (KBQA) focus on a specific underlying knowledge base either because of inherent assumptions in the approach, or because evaluating it on a different knowledge base requires non-trivial changes. However, many popular knowledge bases share similarities in their underlying schemas that can be leveraged to facilitate generalization across knowledge bases. To achieve this generalization, we introduce a KBQA framework based on a 2-stage architecture that explicitly separates semantic parsing from the knowledge base interaction, facilitating transfer learning across datasets and knowledge graphs. We show that pretraining on datasets with a different underlying knowledge base can nevertheless provide significant performance gains and reduce sample complexity. Our approach achieves comparable or state-of-the-art performance for LC-QuAD (DBpedia), WebQSP (Freebase), SimpleQuestions (Wikidata) and MetaQA (Wikimovies-KG).

==> sections/architecture.tex <==
\section{Proposed Architecture}


The KBQA task involves finding an answer in a given Knowledge Graph $\mathcal{G} ; <V, E>$ for a natural question $q$. We consider the setting where a structured query exists that can retrieve the correct answer(s) is present in the KG, and we solve the task by learning a distribution over \sparql{}s to find the correct structured query that would retrieve the required answers, i.e, $$Pr(\sparql | q, G)$$


In this work, we aim to create a learning-based system that generalises across different KBQA datasets built of multiple knowledge bases such as DBpedia, Wikidata, and Freebase. 
% This includes the query graph structure, \sparql operators (\textsc{SELECT}, \textsc{ASK}, etc.), as well as entity and relation linking.
%The required output for any KBQA system is a KG-aligned subgraph that can be executed. 
First, we identify the aspects of KBQA models that can be made generalizable with respect to different KGs, and the parts more strongly tied to the KG.  

Efforts to achieve KG or dataset migration and mapping often involve an automated stage, followed by human curation to refine and make necessary modifications [CITE]. The very existence of an automatic stage is only possible because of similarities shared across them that can be exploited. We make these explicit with the following observation:

The identification of 1-1 mapping between many entities or relations across KGs indicates that granularity and representational choices can be similar. This in turn suggests that for some questions, the query graph structure as a whole could be similar, if not the same. 
Consequently, a learning system trained on a QA dataset on one KG could , if designed in a manner that facilitates transfer.

% \begin{enumerate}
%     \item Query graph structures between different KGs share many similarities. In Table \ref{tab:sketch}, the body of the \sparql query is exactly the same across KGs; 2 triples, V-shaped (join on ?var) with the same directionality.
%     \item Relations across KGs generally share semantic meaning as well as lexical similarities. In Table \ref{tab:sketch}, the relation label for a movie director is \textit{director} in DBpedia, \textit{ directed by} in WikiMovies and \textit{director} in Wikidata. The same behaviour can be seen for \textit{language} relation.
% \end{enumerate}

An example illustrating the above observation is shown in Table \ref{tab:sketch}, for the question \textit{The films directed by John Krasinski are in which language?}. The body of the \sparql query is exactly the same across KGs; 2 triples, V-shaped (join on ?var) with the same directionality. Relations across KGs generally share semantic meaning as well as lexical similarities.
% In light of this example,

% \begin{enumerate}
%     \item Query graph structures between different KGs share many similarities. For instance, answering ``Who is no. 1 in golf?'' involves the same set query constructs (\textsc{SELECT}, \textsc{ORDER BY}, and \textsc{LIMIT}) across KGs. 
%     % While there are \textit{differences} in representation across KGs (eg. Refication, present in Wikidata but not DBPedia), they also share many representational choices. 
%     Similarly, across KGs, a relation's subject often appears in the head of the triple, and object appears as the tail. Granularities of relations often match as well, meaning there are often 1-1 correspondences between certain relations across KGs. \todo{add examples of such relations}
%     \item Relations across KGs generally share semantic meaning as well as lexical similarities. eg. dbo:author, dbp:author, Writer, http://rdf.freebase/fiction.book.writer, etc. Partial relation linking, i.e, identifying likely relation surface forms, can generalize well across KGs. For complete relation linking, we would need to further disambiguate the surface forms to actual KG relations (eg. dbo:author vs dbp:author).\\ 
    
% \end{enumerate}



% there are multiple similarities across KGs if we ignore the entities and consider only some semantically meaningful surface forms of the relations: \\

% \begin{table}[]
% % \resizebox{\linewidth}{!}{
% \small
% \centering
% \begin{tabular}{c|c|c}
% \toprule
% DBpedia & MetaQA-KG & Wikidata \\
% \midrule 
% \begin{minipage}{1.8in}
% \begin{verbatim}
% ?var <director> <entity>
% ?var <language> ?ans
% \end{verbatim}
% \end{minipage}
% &        
% \begin{minipage}{2in}
% \begin{verbatim}
% ?var <directed by> <entity>
% ?var <In language> ?ans 
% \end{verbatim}
% \end{minipage}
% &         
% \begin{minipage}{2in}
% \begin{verbatim}
% ?var <director> <entity>
% ?var <original language of film> ?ans
% \end{verbatim}
% \end{minipage}
% \\
% \bottomrule
% \end{tabular}
% % }
% \label{tab:sketch}
% \caption{Query sketch for the question ``The films directed by John Krasinski are in which language?"}
% \end{table}


\begin{table}[]
% \resizebox{\linewidth}{!}{
% \small
\centering
\begin{tabular}{c|c}
\toprule
KG & Query Graph Structure \\
\midrule 
DBpedia
&
\begin{minipage}{3in}
\small
\begin{verbatim}
?var <director> <entity>
?var <language> ?ans
\end{verbatim}
\end{minipage} \\    
\midrule
MetaQA-KG
&
\small
\begin{minipage}{3in}
\begin{verbatim}
?var <directed by> <entity>
?var <In language> ?ans 
\end{verbatim}
\end{minipage} \\
\midrule
Wikidata
&
\small
\begin{minipage}{3in}
\begin{verbatim}
?var <director> <entity>
?var <original language of film> ?ans
\end{verbatim}
\end{minipage}
\\
\bottomrule
\end{tabular}
% }
\label{tab:sketch}
\caption{Query sketch for the question ``The films directed by John Krasinski are in which language?"}
\end{table}

% DBpedia : \\
% \begin{verbatim}
%     ?var <director> <entity>
%     ?var <language> ?ans
% \end{verbatim}
% ?var --director-- <entity> \\
% ?var --language-- ?ans \\
% MetaQA : \\
% ?var --directed by-- <entity> \\
% ?var --In language-- ?ans \\

Therefore, we propose a 2-stage architecture that explicitly separates query sketch generation (\textit{semantic parsing stage}), which transfers across KGs/datasets, and \textit{KG interaction} to find the answer, which is tied to the specific KG in question.

% the (a) semantic parsing of the query (which transfers across KGs/datasets), and (b) KG interaction to find the answer, which is tied to the specific KG in question.


The semantic parsing stage includes query structure generation, \sparql operator selection, and partial relation linking. We call the output of this stage a \textit{softly-tied} semantic parse, because the query structure adheres to a given KG's schema, and the relation surface forms are obtained from the given KG's relations; and yet the learnt parameters can transfer across KGs. 

% While some systems do use a generic NLP semantic parser \cite{kapanipathi2020question}, there can be mismatches between this semantic parse and the required KG subgraph (Additional nodes/edges, granularity, etc.). Our softly-tied semantic parse, in contrast, is already in the KG structure, meaning each node corresponds to either one or a set of entities, and each edge corresponds to some relation in our KG. 

In the second stage, we bind it strongly to the KG, by (a) resolving the textual relations into specific KG relations, (b) resolving the entities using an Entity Linker, as well as (c) rank the obtained semantic parses based on actual sub-graphs present in the KG. 
% In future work, we plan to modify this stage to utilize an embeddings-based approach to evaluate the semantic parses obtained in the incomplete setting, as in [CITE EmbedKGQA]. 


Formally, we decompose the SPARQL into a skeleton $S : (V_S, E_S) $. We are required to find an edge to KG relation mapping $f_R : E_S \longrightarrow E$ and a node to KG entity mapping $f_E : V_S \longrightarrow V$. For the Knowledge Graph $\mathcal{G} : (V, E, V_{text}, E_{text})$ with text labels or descriptions corresponding to the entities $V$ and relations $E$, we can express the mapping of $V_S, E_S$ to $V, E$ through this intermediary textual space.
We learn an edge to relation text mapping $f_R' : E_S \longrightarrow E_{text}$ as well as a node to entity text mapping
$f_E' : V_S \longrightarrow V_{text}$ instead, yielding:


\begin{align*}
 Pr(\sparql | q, G)  &= Pr(S, f_R, f_E | q, G) \\
 &\sim \underbrace{Pr(S, f_R', f_E' | q, G)}_\text{Stage I}  . \underbrace{Pr(S, f_R, f_E | S, f_R', f_E', G)}_\text{Stage II}
\end{align*}

\begin{figure}[]
    \centering
    \includegraphics[width=0.7\textwidth]{Images/NeurIPS_arch}
    \caption{Semantic Parsing}
    \label{fig:arch}
\end{figure}

\subsection{Semantic Parsing}

The input to this stage is a question, and a list of relation-surface forms from the underlying KG. The required output, a softly-tied semantic parse, consists of skeleton generation and partial relation linking.
These steps are described below:

\textbf{Skeleton Generation:}
First, the question is passed to a \textsc{Seq2Seq} model, a transformer-based Encoder-Decoder setup \cite{}, that is trained to produce a \sparql skeleton. 
An example of a \sparql skeleton for our running example ``The films directed by John Krasinski are in which language?" is as follows: \\ \\
{\small
\centerline{\texttt{SELECT ?var0 WHERE \{ ?var1 :prop0 :ent0. ?var1 :prop1 ?var0 . \}}}
}

The skeleton captures the \sparql operators needed to answer the question; i.e. \ask, \select, \countsparql  or \filter,  as well as the query graph structure, with placeholder nodes for entities (e.g. \texttt{:ent0}) and relations (e.g. \texttt{:prop0}). For many types of questions, the generated \sparql skeletons for different KGs are similar. Structural characteristics unique to a KG (eg. reification or granularity mismatches between KGs) are learnt when fine-tuning the skeleton generation on a dataset that uses that KG. A query skeleton $S_0$ is generated that comprises only of \sparql primitives and a pre-defined set of entity and relation placeholders. All knowledge base's instantiates (i.e. specific entities and relations) are replaced by the corresponding placeholder as shown in the example skeleton above.

Formally, Let $(S, E, R)$ be the decomposed \sparql query, where $S_0 = [s_1 ...s_T]$ with some $s_i$ being \sparql operators in $\mathcal{V}_0$ and some $s_j$ being placeholders in $\mathcal{V}_0^+ \subset \mathcal{V}_0$. We define $E: \{s_j \xrightarrow{} e_x; e_x \in \mathcal{E}\}$ and $R: \{s_j \xrightarrow{} r_y; r_y \in \mathcal{R}\}$ to be the mappings from the placeholders to the actual KB instances. 


We employ a neural \texttt{Seq2Seq} model as our skeleton generator. Given $\mathcal{V} = \{w_1, ..., w_M\}$ is a vocabulary of tokens, the question $\mathbf{q} = [w_1 ...w_{|q|}]$ is a sequence of tokens $w_i \in \mathcal{V}$. We first represent the question using a pre-trained Transformer encoder, more specifically

% \begin{align*}
% \mathbf{h}_{[CLS]}^{(l)}, \ldots, \mathbf{h}_{i}^{(l)}, \ldots, \mathbf{h}_{|q|}^{(l)}, \mathbf{h}_{[SEP]}^{(l)}=\texttt{Transformer}\left(\left\{[CLS], w_{1}, \ldots, w_{|q|}, [SEP] \right\}\right)
% \end{align*}

\begin{align*}
    \textsc{Bert}(\mathbf{q}) &= [\textsc{Cls}] \text{ } \mathbf{q} \text{ } [\textsc{Sep}]\\
    \textsc{Embed}_{\text{input}}(\mathbf{q}) &= \mathbf{W}_{\text{input }} \textsc{Bert}_{\text {CLS }}\left(\textsc{Bert }(\mathbf{q})\right)
\end{align*}

We then use a transformer decoder with attention mechanism. 
The decoder consumes the encoder states and produces a distribution over possible \sparql operators in $\mathcal{V}_0$.
% At each decoding step, the decoder takes in its previous hidden state, uses it as the query to compute attention weights over the encoder states, formulates a decoder context. 
% This decoder context is then combined with the embedding of the previous step's operator to form the input to the decoder's LSTM cell. 
% We utilize teacher forcing, feed in ground-truth operators with some probability $p$ over the course of training. 

\begin{align*}
\mathbf{u}_{i} &= \texttt{Transformer}\left(\left\{\mathbf{h}^{L}_{[CLS]}, \ldots, \mathbf{h}^{L}_{i-1} \right\}\right)\\ \mathbf{\hat{y}}_i &=\texttt{Softmax}(\texttt{FNNLayers}(\mathbf{u}_{i}))
\end{align*}

The output of each decoding step is a softmax over possible operators $s_i \in \mathcal{V}_0$. In a naive \texttt{Seq2Seq} settings, $\mathcal{V}_0$ would comprise not only \sparql pre-defined primitives, but also all knowledge base entities and relations, yielding a label space with size $|\mathcal{V}_0| = (\texttt{Const} + |\mathcal{E}| + |\mathcal{R}|)$, which is proportional to the size of the knowledge base. Therefore, we first generate a query skeleton, effectively reduce $|\mathcal{V}_0|$ to a manageable constant; but more importantly allows generalization across KGs. The next step to obtain a softly-tied semantic parse is to perform partial relation linking.

% \june{@Srini if this step isn't in the current implementation, then we can drop it.}
% Having a smaller label space, we also enjoy the benefits of modeling the global structure of the query. In particular, we apply a CRF layer over the output sequence $\mathbf{\bar{Y}}$ to exploit the constraints $\Gamma$ between \texttt{SPARQL} operators, such as \texttt{SELECT} must be followed by \texttt{DISTINCT} or a list of variables \texttt{?varX}.

% \begin{equation}
%     Pr(S_0 \mid q) = \frac{1}{Z(\mathbf{y})} Pr(y_i \mid q) Pr(y_i, y_j \mid q, \Gamma)
% \end{equation}

\textbf{Partial Relation Linking:}
We then identify the relation surface forms that correspond to the relation placeholders in the \sparql skeleton (\texttt{:prop0}, \texttt{:prop1}, etc.) 
In each KG, we first map the relations to their respective surface forms, using either \textit{label} relations from the KG itself, or by extracting some semantically meaningful surface form from the relation URL. This mapping can be many-to-one. Table \ref{tab:rel2surface} shows few examples. 

\begin{table}[h!]
\centering
\begin{tabular}{c|c|c}
\toprule
 KG & KG Relation & Derived Surface Form \\
\midrule
\multirow{3}{*}{DBpedia}    &      dbo:language     &    language \\
            &  dbp:language & language \\
            &  dbp:languages &   languages  \\

\midrule
\multirow{2}{*}{Wikidata}    &  P397  & official language     \\
                             &  P364  & original language of film or TV show  \\
\midrule
\multirow{3}{*}{FreeBase} & people.ethnicity.languages\_spoken & languages spoken\\
& location.country.languages\_spoken &  languages spoken\\
& film.director.film & film\\
\bottomrule
\end{tabular}
\caption{Examples for mapping relations to their surface forms. Note that this can be noisy.}
\label{tab:rel2surface}
\end{table}


As noted before, these surface forms across KGs often have semantic and lexical similarity.
We wish to identify which relation surface form best matches each relation placeholder in the skeleton. We thus train the decoder and relation encoder to project into the same space. Concretely, the decoder state corresponding to each relation placeholder is optimized to be closest to the encoded representation of the correct relation. In Figure \ref{fig:arch}, the encoded representation for "Directed by" is closest to the decoder state for \texttt{:prop0}.


% Hence, we opt instead to produce a ranked list of candidate interpretations that are \textit{almost} SPARQLS in KG vocabulary, but not strictly so. Specifically, the relations are still in textual form. This trick allows transfer not only question syntax across QA datasets, but also schemas that are common across popular KGs. Note that this SPARQL-like structure is not yet executable since the same surface form can map to multiple relations in the actual KG. In KGs like DBPedia, this occurs due to namespace differences (\textit{dbo:author} vs \textit{dbp:author}); and in FreeBase, though we find that ignoring the full domain of the relation reduces noise and improves relation encoding on average, conflicts occur in some cases (like \textit{winner} mapping to both \textit{election.winner} and \textit{race.winner}). 



\subsection{KG Interaction}

The \sparql skeleton together with the partial relation linking produces a ranked list of softly-tied semantic parses. 
Sometimes this phase produces multiple semantic interpretations, either due to noisy surface forms or due to the presence of distinct but similar-looking relations in the KG.  
In the running example, \textit{``The films directed by John Krasinski are in which language?"}, the first stage produces: \\

\begin{verbatim}
            P=0.87    SELECT ?var0 where { 
                        ?var1 director :ent0. 
                        ?var1 language ?var0.}  
            P=0.76    SELECT ?var0 where {
                        ?var1 director :ent0. 
                        ?var1 languages ?var0.} 
                               .
                               .
                               .
\end{verbatim}

% Each relation surface form can map to one or more actual KG relations, implying that each soft semantic parse produces

Given a list of possible semantic parses, the KG interaction stage performs the following steps to produce the final question answer: 1) disambiguate relations' textual form and and link it to the specific KG relations, 2) link the different entities to their corresponding placeholders in the skeleton and 3) select the correct \sparql based on the actual facts in the KG.

For entity linking, we leverage pre-trained off-the-shelf Entity Linker, BLINK \cite{wu2019zero}, to obtain entity mentions in the question and their corresponding linked entities based on the specific KG. In the example above, `John Krasinski' which corresponds to \smalltt{:ent0} will be linked to \smalltt{dbr:John\_Krasinski} in DBpedia, or \smalltt{wd:Q313039} in Wikidata. 
% We use gold entities when comparing against other systems that do so. The entity placeholders are thus filled with the appropriate entity. 

Recall from Table \ref{tab:rel2surface} that each surface form in a semantic parse can map to one or more KG relations. In practise, we find that most relation surface forms map to not more than 3 KG relations. Thus, each softly-tied semantic parse produces one or more fully executable \sparql{}s, and we simply choose the highest-ranked \sparql{} that also exists in the KG to produce the answer.

Consider that we wish to answer our running example in DBpedia. In the example above, assume ``director" maps to [\texttt{dbo:director}, \texttt{dbp:director}]. ``language" maps to [\texttt{dbo:language}] and ``languages" maps to [\texttt{dbp:languages}].

Thus, the 2 semantic parses above produce the following 4 \sparql{}s:


\begin{table}[h!]
\centering
\begin{tabular}{c|c}
\toprule
Rank & Predicted SPARQL Query \\
\midrule 
1
&
\begin{minipage}{3in}
\small
\begin{verbatim}
SELECT ?var0 where { 
    ?var1 dbo:director dbr:John_Krasinski.
    ?var1 dbo:language ?var0. }  
\end{verbatim}
\end{minipage} \\    
\midrule
1
&
\small
\begin{minipage}{3in}
\begin{verbatim}
SELECT ?var0 where { 
    ?var1 dbp:director dbr:John_Krasinski. 
    ?var1 dbo:language ?var0. } 
\end{verbatim}
\end{minipage} \\
\midrule
2
&
\small
\begin{minipage}{3in}
\begin{verbatim}
SELECT ?var0 where { 
    ?var1 dbo:director dbr:John_Krasinski. 
    ?var1 dbp:languages ?var0. }  
\end{verbatim}
\end{minipage}
\\
\midrule
2
&
\small
\begin{minipage}{3in}
\begin{verbatim}
SELECT ?var0 where { 
    ?var1 dbp:director dbr:John_Krasinski. 
    ?var1 dbp:languages ?var0. }  
\end{verbatim}
\end{minipage}
\\
\bottomrule
\end{tabular}
% }
\label{tab:sketch}
\caption{Top predicted SPARQL queries for the question ``The films directed by John Krasinski are in which language?"}
\end{table}

We choose the highest ranked \sparql whose subgraph exists in the KG. Ties are broken by arbitrarily.

% \centerline{\texttt{SELECT ?var0 where \{?var1 dbo:director dbr:John\_Krasinski. ?var1 dbo:language ?var0.\} 0.87}}
% \centerline{\texttt{SELECT ?var0 where \{?var1 dbp:director dbr:John\_Krasinski. ?var1 dbo:language ?var0.\} 0.87}} 
% \centerline{\texttt{SELECT ?var0 where \{?var1 dbo:director dbr:John\_Krasinski. ?var1 dbp:languages ?var0.\} 0.76 }}
% \centerline{\texttt{SELECT ?var0 where \{?var1 dbp:director dbr:John\_Krasinski. ?var1 dbp:lanugages ?var0.\} 0.76 }}




% During training, skeletons that have entity placeholders corresponding to the order in which entity mentions appear in the question text. Concretely, the entity corresponding to the first mention is replaced by \texttt{:ent0}, second entity is replaced by \texttt{:ent1}, and so on. 

% Transformer encoders such as BERT easily capture the positional and Named Entity information present in the question, learning to produce skeletons with the same ordering. Thus entities which makes the replacement of entity placeholders during inference very simple. All detected entities are 




% The KG interaction stage is thus responsible for (a) Converting each soft semantic parse into one or more resolved semantic parses. (b) Evaluating the best resolved semantic parse, based on the KG. 

% Softly-tied semantic parse : Entities are not linked, and relations remain in textual form. \\
% Strictly-tied semantic parse : Relation surface forms are mapped to an actual KG relation, and entities are linked and filled in the soft semantic parse. This is a SPARQL that can be executed.




% The semantic parsing is still in the vocab


% We propose a two-steps, multi-tasks learning model for generating the structured query. In the first step, we generate a query \textit{skeleton} $S_0$ that comprises only \texttt{SPARQL} \textit{primitives} and a pre-defined set of \textit{entity and relation placeholders}. All knowledge base's instantiates (i.e. specific entities and relations) are replaced by the corresponding \textit{placeholder} as shown in Figure \ref{fig:sparql_decomp}. 
% We later show that this step significantly reduces the size of label space of $S$ and allows a more effective learning objective in Section ?. Moving on to the second step, we employ several KB-related learning objectives to find out entities and relations that best fit into the placeholders in the previous step (Section ?).
% % By doing so, we effectively reduce the label space of $S$ do

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{kbqa/SPARQL_decomp.png}
%     \caption{A \texttt{SPARQL} query decomposed into a skeleton and filling labels.}
%     \label{fig:sparql_decomp}
% \end{figure}

% Let $S = (S_0, E, R)$ be the decomposed \texttt{SPARQL} query, where $S_0 = [s_1 ...s_T]$ with some $s_i$ being \texttt{SPARQL} operators in $\mathcal{V}_0$ and some $s_j$ being placeholders in $\mathcal{V}_0^+ \subset \mathcal{V}_0$. We define $E: \{s_j \xrightarrow{} e_x; e_x \in \mathcal{E}\}$ and $R: \{s_j \xrightarrow{} r_y; r_y \in \mathcal{R}\}$ to be the mappings from the placeholders to the actual KB instances. We decompose $Pr(S \mid q, \mathcal{G})$ into a \textit{skeleton generating} step and a \textit{skeleton filling} step, yielding

% \begin{equation}
%     Pr(S \mid q, \mathcal{G}) = Pr(S_0 \mid q) Pr(E \mid q, \mathcal{G}, S_0) Pr(R \mid q, \mathcal{G}, S_0)
% \end{equation}
% % \jaylee{Are the E, R probabilities drawn separately? Why are they modeled to be conditionally independent?} \\

% \subsection{Skeleton generating step.} 
% We employ a neural \texttt{Seq2Seq} model as our skeleton generator. Given $\mathcal{V} = \{w_1, ..., w_M\}$ is a vocabulary of tokens, the question $\mathbf{q} = [w_1 ...w_L]$ is a sequence of tokens $w_i \in \mathcal{V}$. We first represent the question using a pre-trained Transformer encoder, more specifically

% \begin{align*}
% \mathbf{X}^{0} &=\texttt{TokenEmbed}(\mathbf{q}) \\
% \mathbf{X}^{1} &=\texttt{Transformer}(\mathbf{X}^{0}, \texttt{ num\_layers } = l_{0}) \\
% \mathbf{X}^{2} &=\texttt{TransformerPooler}(\mathbf{X}^{1})
% \end{align*}

% We then use a transformer decoder with attention mechanism. The decoder consumes the encoder states and produces a distribution over possible \texttt{SPARQL} operators in $\mathcal{V}_0$. At each decoding step, the decoder takes in its previous hidden state, uses it as the query to compute attention weights over the encoder states, formulates a decoder context. This decoder context is then combined with the embedding of the previous step's operator to form the input to the decoder's LSTM cell. We utilize teacher forcing, feed in ground-truth operators with some probability $p$ over the course of training. 

% \begin{align*}
% \mathbf{C}^{i} &=\texttt{BahdanauAttention}(\mathbf{H}^{i-1}, \mathbf{X}^{1}) \\
% \mathbf{H}^{i} &=\texttt{LSTM}(\mathbf{C}^{i}, \texttt{OperatorEmbed}(\mathbf{\bar{Y}}^{i-1})) \\
% \mathbf{\bar{Y}}^{i} &=\texttt{Softmax}(\texttt{FNNLayers}(\mathbf{H}^{i}))
% \end{align*}

% The output of each decoding step is a softmax over possible operators $s_i \in \mathcal{V}_0$. In a typical \texttt{Seq2Seq} settings, $\mathcal{V}_0$ would comprise not only \texttt{SPARQL} pre-defined primitives, but also all knowledge base entities and relations, yielding a label space with size $|\mathcal{V}_0| = (\texttt{Const} + |\mathcal{E}| + |\mathcal{R}|)$, which is proportional to the size of the knowledge base. Therefore, we propose a two-steps approach that first generates the query skeleton, effectively reduce $|\mathcal{V}_0|$ to a manageable constant. Similar ideas have been explored for Text-to-SQL \june{citations?}. However, our approach is different \june{...}.\\

% Having a smaller label space, we also enjoy the benefits of modeling the global structure of the query. In particular, we apply a CRF layer over the output sequence $\mathbf{\bar{Y}}$ to exploit the constraints $\Gamma$ between \texttt{SPARQL} operators, such as \texttt{SELECT} must be followed by \texttt{DISTINCT} or a list of variables \texttt{?varX}.

% \begin{equation}
%     Pr(S_0 \mid q) = \frac{1}{Z(\mathbf{y})} Pr(y_i \mid q) Pr(y_i, y_j \mid q, \Gamma)
% \end{equation}

% \subsection{Skeleton filling step.} 
% In this step, we propose multi-tasks learning objectives that are jointly trained to fill in the placeholders $s_j \in S_0$ with knowledge base instances. First of all, we present three objectives for predicting placeholder-entity mappings. The \textit{mention detection objective}  finds mention spans in the question that yield entities in the \texttt{SPARQL} query. The \textit{entity linking objective} matches mentions spans to KB entity identifiers. The \textit{entity pointer objective} decides which placeholder goes with which mention span, and thereof which entity identifier. We propose an approach to jointly train these three objectives end-to-end in Section ?. At the same time, we also train a \textit{predicate classifier} to produce KB relation identifiers corresponding to predicate placeholders in the query skeleton. Separating the placeholders filling step into these objectives allows further decoupling of the skeleton decoding step and KB-related tasks. This characteristic of the model gives us several advantages such as having better modularity and stronger training signals for each component. \june{Finally, we propose an in/out-degree beam search to enforce global, multi-hop interrelations in the sub-KB of top-k predicted KB instances.} 

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/intro.tex <==
\section{Introduction}


Knowledge Base Question Answering (KBQA) has gained significant popularity in recent times due to its real-world applications, facilitating the use of rich RDF data stores without the need for technical query-syntax. Given a natural language question, a KBQA system is required to find an answer based on the facts available in a given knowledge graph. For example, given the question \textit{"Who is the director of the film Titanic"}, a KBQA system should retrieve the entity corresponding to "James Cameron". This would be \smalltt{dbr:James\_Cameron}\footnote{dbr: \url{http://dbpedia.org/resource/}} in DBpedia~\cite{auer2007dbpedia}, \smalltt{wd:Q42574}\footnote{wd: \url{http://www.wikidata.org/entity}} in Wikidata~\cite{vrandevcic2014wikidata}, and \smalltt{fb:m.03\_gd}\footnote{fb: \url{http://rdf.freebase.com/ns/}} in Freebase~\cite{bollacker2008freebase}. 


Existing KBQA approaches are typically tuned for a specific underlying knowledge base, and using a different KG may require non-trivial changes to the system.
This is evident when looking at the datasets used to evaluate existing systems (see Table~\ref{tab:existing_eval} for details). With the exception of WDAqua~\cite{diefenbach2017wdaqua}, an early KBQA system, most state-of-the-art approaches focused primarily on one or two KGs.

In this work, we present a novel generalizable KBQA approach that works seamlessly with multiple knowledge graphs. Our approach attempts to separate aspects of KBQA systems that are softly tied to the KG but generalizable, from the parts more strongly tied to a specific KG. Concretely, our approach has two stages: 1) The first stage is a generative model that predicts a query skeleton, which includes the number of constraints in the query, the different operators in it, as well as candidate relations based on label semantics. 2) The second stage converts this softly-tied semantic parse of the question to a final query (with entity and relation linking based on the structure of the KG) that can be evaluated on the underlying knowledge graph to retrieve the final answer. With this simple architecture, our approach demonstrates state-of-the-art or comparable performance on datasets across four different knowledge graphs: LC-QuAD (DBpedia), WebQSP (Freebase), SimpleQuestions (Wikidata) and MetaQA (MetaQA-KG).


\begin{table*}
\centering
\begin{tabular}{l|c|c|c|c} 
\toprule
                               & DBpedia & Wikidata & Freebase & MetaQA-KG  \\ 
\midrule
NSQA~\cite{kapanipathi2020question}          &   \checkmark      &          &          &                                  \\
gAnswer~\cite{zou2014natural}       &    \checkmark     &          &          &                                  \\
QAMP~\cite{vakulenko2019message}          &  \checkmark       &          &          &                                  \\
WDAqua~\cite{diefenbach2017wdaqua}        &    \checkmark     &   \checkmark       &     \checkmark     &              \\
Slot Matching~\cite{maheshwari2019learning} &   \checkmark      &          &          &                                  \\
PullNet~\cite{sun2019pullnet}       &         &          &   \checkmark       &    \checkmark                              \\
EmbedKGQA~\cite{embedkgqa}     &         &          &    \checkmark      &       \checkmark                           \\ 
\midrule
Our Approach                   &    \checkmark     &    \checkmark      &    \checkmark      & \checkmark             \\
\bottomrule
\end{tabular}
\caption{Knowledge Graphs used for evaluation in recent KBQA systems}
\label{tab:existing_eval}
\end{table*}

% While Entity Linking and Relation Linking have been traditionally thought of as KG-specific tasks, recent works (BLINK) have shown that representing entities purely as text allows for transfer across KGs (zero-shot linking). We leverage the similar principles to make relation linking and skeleton generation a KG-tied task while still maintaining transferability. Concretely, we express representations 

In particular, our list of contributions are:

\begin{itemize}
    \item A simple \seqseq architecture for KBQA that separates aspects of the output that are generalizable across KGs, from those that are strongly tied to a specific KG structure. This separation allows transfer learning across different KGs.
    \item To the best of our knowledge, our approach is the first to evaluate on and achieve state-of-the-art or comparable performance on KBQA datasets corresponding to four different knowledge graphs. With our architecture, we show how pre-training can result in performance gains across different underlying KGs.
    % \item We also show that 2 popular multi-hop QA datasets do not test generalizability to unseen combinations of seen relations.
\end{itemize}
% Efforts to achieve KG or dataset migration and mapping often involve an automated stage, followed by human curation to refine and make necessary modifications [CITE]. The very existence of an automatic stage is only possible because of similarities shared across them that can be exploited. We make these explicit with the following observation:

%\noindent KG Setting: Complete KGQA data: Complex queries (multi hop)

% True complex QA must involve evaluating a system's ability to answer unseen combinations of seen relations, i.e,  \textit{compositionality}.


% The trend of deep learning~\cite{}, particularly the transformer based models~\cite{} has significantly improved the accuracy on KGQA datasets. Such models typically of depend on two types of training data (a) question-answer pairs; or (b) question-query pairs.  

% \begin{table}[]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|cc|c|c}
% \toprule

%      & \multicolumn{2}{c|}{DBPedia} & \multicolumn{2}{c|}{WikiData}  & \multicolumn{1}{c|}{Freebase} & WikiMovies \\
% \midrule
%      & QALD     & LC-QuAD 1.0    & SimpleQuestions & LC-QuAD 2.0 & WebQSP                       & MetaQA     \\
% \midrule
% NSQA~\cite{kapanipathi2020question} &   \checkmark         &   \checkmark & &   &  &            \\
% gAnswer~\cite{zou2014natural} &   \checkmark         &  & &   &  &            \\
% QAMP~\cite{vakulenko2019message} &          &   \checkmark & &   &  &            \\
% WDAqua~\cite{diefenbach2017wdaqua} &     \checkmark      &   \checkmark & \checkmark&   & \checkmark &            \\
% Slot Matching~\cite{maheshwari2019learning}   &   \checkmark         &   \checkmark & &   &  &            \\
% PullNet~\cite{sun2019pullnet} &           &  & &   & \checkmark &  \checkmark       \\
% EmbedKGQA~\cite{embedkgqa} &           &  & &   & \checkmark &  \checkmark       \\
% \midrule
% Our Approach &  \checkmark        &   \checkmark & \checkmark&  \checkmark & \checkmark &    \checkmark        \\ 

% \bottomrule
% \end{tabular}
% }
% \caption{Datasets and knowledge graphs used for evaluation in recent KBQA systems}
% \label{tab:existing_eval}
% \end{table}



% \usepackage{booktabs}





% \begin{itemize}
% \item Having an option for semantic parsing provides interpretability and ability to not train with data that are temporally irrelevant. For example -- Who is the president of the United States of America. Hence we focus on models that generate SPARQL queries
% \item Most KBQA approaches have the following drawbacks (a) they are trained on specific knowledge graphs and show significant performance gains on datasets that are built for that specific KG and rarely performing well for other knowledge graphs (b) datasets, in particular the combination of relationships from the KG necessary to answer the question becomes an artifact that can be easily captured by such approaches. Addressing both of the above mentioned challenges encourages models to be genralizable to datasets and knowledge bases.
% \end{itemize}

% In this work, we present a novel generalizable KGQA approach that works seamlessly with multiple knowledge graphs and do not overfit for relations bla bla. 

%\noindent KG Setting: Complete KGQA data: Complex queries (multi hop)

% True complex QA must involve evaluating a system's ability to answer unseen combinations of seen relations, i.e,  \textit{compositionality}.

% Possible Contributions:
% \begin{enumerate}
%     % Analysis done - Show large drop in performance on the special subet, as well as 0%, 3% analysis by Nandana
%     \item Flaw in 2 ``multi-hop" datasets. Repetition of seen combinations - Assertion: Not actually complex QA. Propose a new dataset split with unseen combinations of seen relations - WebQSP and MetaQA.
    
%     % First system to be evaluated and achieve SOTA on multiple multi-hop datasets from different KGs, intermediate form is as close to SPARQL as possible, while still retaining generalizability. 
%     % @Srini 1. Need to provide evidence for KG transfer (say increased Hits@1) on one QA dataset after training embeddings on another QA dataset. Relations must overlap for this. Evidence-Train embeddings on lcquad2.0, test on SimpleQuestions-wiki. @Srini 2. Prove assertion of QA having greater inductive bias because of closed-world assumption. Evidence-In MetaQA, train using closed and open world assumption, check which is higher.
%     % \item The method and motivation for fine-tuning KG embeddings using multi-hop QA data. The derivation of \textit{relation composition} functions for some popular link prediction scoring functions, to do the above. If possible, show embeddings-based KG interaction \textit{also} transfers across multiple datasets for the same KG.
%     \item Architecture that separates the semantic parsing and KG interaction steps; such that Semantic parsing transfers across datasets. involves: A simple seq2seq baseline that explicitly recognizes the decomposed relations of the question using KB vocabulary (eg. the SPARQL), and then chooses the top predicted query that exists in the KG. 
%     % does standard link prediction using the above fine-tuned embeddings to obtain the answer.
 
% \end{enumerate}


==> sections/introduction_pavan.tex <==
\section{Introduction}


Knowledge Base Question Answering (KBQA) has gained significant popularity in recent times due to its real-world applications, facilitating the access to rich knowledge graphs  without the need for technical query-syntax. The task is, given a natural language question, a KBQA system is required to find an answer based on the facts available in the knowledge graph. For example, given the question \textit{"Who is the director of the film Titanic"}, a KBQA system should retrieve the entity corresponding to "James Cameron". This would be \smalltt{dbr:James\_Cameron}\footnote{dbr: \url{http://dbpedia.org/resource/}} in DBpedia~\cite{auer2007dbpedia}, \smalltt{wd:Q42574}\footnote{wd: \url{http://www.wikidata.org/entity}} in Wikidata~\cite{vrandevcic2014wikidata}, and \smalltt{fb:m.03\_gd}\footnote{fb: \url{http://rdf.freebase.com/ns/}} in Freebase~\cite{bollacker2008freebase}. 

%With the exception of MetaQA~\cite{}, KBQA techniques have primarily focused on open knowledge graphs such as  Freebase~\cite{}, Wikidata~\cite{}, and DBpedia~\cite{}. 

KBQA has been evaluated on multiple different knowledge graphs such as Freebase~\cite{bollacker2008freebase}, Wikidata~\cite{vrandevcic2014wikidata}, DBpedia~\cite{auer2007dbpedia}, and MetaQA~\cite{}. Most existing heuristic-based KBQA approaches are typically tuned for a specific underlying knowledge base making it non-trivial to generalize and adapt it to other knowledge graphs. For instance, NSQA~\cite{kapanipathi2020question}, gAnswer~\cite{zou2014natural}, and QAMP~\cite{vakulenko2019message} which are the best approaches on DBpedia-based datasets requires most modules such as entity and relation linking to adapt to a new knowledge graph. On the other hand, system such as WDAqua~\cite{diefenbach2017wdaqua} that intended focus on generalizability shows reduced performance on each of the datasets.

Recently there is a surge in end-to-end learning approaches such as PullNet~\cite{sun2019pullnet} and EmbedKGQA~\cite{embedkgqa} that show some generalizability with evaluation on two knowledge graphs. These techniques, however, are highly sensitive to the training data. For instance, EmbedKGQA shows a significant drop (99\%-50\%) in performance on relation compositions that are not seen during training, hence impacting its ability to generalize over new  compositions of relations. In summary, existing approaches face challenges to generalize over knowledge graphs or over unseen relation compositions.


%%% Justify both here 
%% a. Two step approach with softly aligned parse which allows generalizability between knowledge graphs. 
%% b. the softly aligned semantic parse decomposes relations and learns predicting single relations and not combinations from the training data. This facilitates predicting new combinations (more technical). 
In this work, we present a novel generalizable KBQA approach that works seamlessly with multiple knowledge graphs. Our approach attempts to separate aspects of KBQA systems that are softly tied to the KG but generalizable, from the parts more strongly tied to a specific KG.  Concretely, our approach has two stages: 1) The first stage is a generative model that predicts a query skeleton, which includes the number of constraints in the query, the different operators in it, as well as candidate relations based on label semantics. 2) The second stage converts this softly-tied semantic parse of the question to a final query (with entity and relation linking based on the structure of the KG) that can be evaluated on the underlying knowledge graph to retrieve the final answer. \pavan{improve this paragraph by addressing the two challenges and how they are addressed.}


\begin{table*}
\centering
\begin{tabular}{l|c|c|c|c} 
\toprule
                               & DBpedia & Wikidata & Freebase & MetaQA-KG  \\ 
\midrule
NSQA~\cite{kapanipathi2020question}          &   \checkmark      &          &          &                                  \\
gAnswer~\cite{zou2014natural}       &    \checkmark     &          &          &                                  \\
QAMP~\cite{vakulenko2019message}          &  \checkmark       &          &          &                                  \\
WDAqua~\cite{diefenbach2017wdaqua}        &    \checkmark     &   \checkmark       &     \checkmark     &              \\
Slot Matching~\cite{maheshwari2019learning} &   \checkmark      &          &          &                                  \\
PullNet~\cite{sun2019pullnet}       &         &          &   \checkmark       &    \checkmark                              \\
EmbedKGQA~\cite{embedkgqa}     &         &          &    \checkmark      &       \checkmark                           \\ 
\midrule
Our Approach                   &    \checkmark     &    \checkmark      &    \checkmark      & \checkmark             \\
\bottomrule
\end{tabular}
\caption{Knowledge Graphs used for evaluation in recent KBQA systems}
\label{tab:existing_eval}
\end{table*}

% While Entity Linking and Relation Linking have been traditionally thought of as KG-specific tasks, recent works (BLINK) have shown that representing entities purely as text allows for transfer across KGs (zero-shot linking). We leverage the similar principles to make relation linking and skeleton generation a KG-tied task while still maintaining transferability. Concretely, we express representations 

Our contributions are as follows:

\begin{itemize}
    \item A simple \seqseq architecture for KBQA that separates aspects of the output that are generalizable across KGs, from those that are strongly tied to a specific KG structure. This separation allows transfer learning across different KGs.
    \item To the best of our knowledge, our approach is the first to evaluate on and achieve state-of-the-art or comparable performance on KBQA datasets corresponding to four different knowledge graphs, i.e, LC-QuAD (DBpedia), WebQSP (Freebase), SimpleQuestions (Wikidata) and MetaQA (MetaQA-KG). With our architecture, we show how pre-training can result in performance gains across different underlying KGs.
    \item Unseen combinations contributions.
    % \item We also show that 2 popular multi-hop QA datasets do not test generalizability to unseen combinations of seen relations.
\end{itemize}
% Efforts to achieve KG or dataset migration and mapping often involve an automated stage, followed by human curation to refine and make necessary modifications [CITE]. The very existence of an automatic stage is only possible because of similarities shared across them that can be exploited. We make these explicit with the following observation:

%\noindent KG Setting: Complete KGQA data: Complex queries (multi hop)

% True complex QA must involve evaluating a system's ability to answer unseen combinations of seen relations, i.e,  \textit{compositionality}.


% The trend of deep learning~\cite{}, particularly the transformer based models~\cite{} has significantly improved the accuracy on KGQA datasets. Such models typically of depend on two types of training data (a) question-answer pairs; or (b) question-query pairs.  

% \begin{table}[]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|cc|c|c}
% \toprule

%      & \multicolumn{2}{c|}{DBPedia} & \multicolumn{2}{c|}{WikiData}  & \multicolumn{1}{c|}{Freebase} & WikiMovies \\
% \midrule
%      & QALD     & LC-QuAD 1.0    & SimpleQuestions & LC-QuAD 2.0 & WebQSP                       & MetaQA     \\
% \midrule
% NSQA~\cite{kapanipathi2020question} &   \checkmark         &   \checkmark & &   &  &            \\
% gAnswer~\cite{zou2014natural} &   \checkmark         &  & &   &  &            \\
% QAMP~\cite{vakulenko2019message} &          &   \checkmark & &   &  &            \\
% WDAqua~\cite{diefenbach2017wdaqua} &     \checkmark      &   \checkmark & \checkmark&   & \checkmark &            \\
% Slot Matching~\cite{maheshwari2019learning}   &   \checkmark         &   \checkmark & &   &  &            \\
% PullNet~\cite{sun2019pullnet} &           &  & &   & \checkmark &  \checkmark       \\
% EmbedKGQA~\cite{embedkgqa} &           &  & &   & \checkmark &  \checkmark       \\
% \midrule
% Our Approach &  \checkmark        &   \checkmark & \checkmark&  \checkmark & \checkmark &    \checkmark        \\ 

% \bottomrule
% \end{tabular}
% }
% \caption{Datasets and knowledge graphs used for evaluation in recent KBQA systems}
% \label{tab:existing_eval}
% \end{table}



% \usepackage{booktabs}





% \begin{itemize}
% \item Having an option for semantic parsing provides interpretability and ability to not train with data that are temporally irrelevant. For example -- Who is the president of the United States of America. Hence we focus on models that generate SPARQL queries
% \item Most KBQA approaches have the following drawbacks (a) they are trained on specific knowledge graphs and show significant performance gains on datasets that are built for that specific KG and rarely performing well for other knowledge graphs (b) datasets, in particular the combination of relationships from the KG necessary to answer the question becomes an artifact that can be easily captured by such approaches. Addressing both of the above mentioned challenges encourages models to be genralizable to datasets and knowledge bases.
% \end{itemize}

% In this work, we present a novel generalizable KGQA approach that works seamlessly with multiple knowledge graphs and do not overfit for relations bla bla. 

%\noindent KG Setting: Complete KGQA data: Complex queries (multi hop)

% True complex QA must involve evaluating a system's ability to answer unseen combinations of seen relations, i.e,  \textit{compositionality}.

% Possible Contributions:
% \begin{enumerate}
%     % Analysis done - Show large drop in performance on the special subet, as well as 0%, 3% analysis by Nandana
%     \item Flaw in 2 ``multi-hop" datasets. Repetition of seen combinations - Assertion: Not actually complex QA. Propose a new dataset split with unseen combinations of seen relations - WebQSP and MetaQA.
    
%     % First system to be evaluated and achieve SOTA on multiple multi-hop datasets from different KGs, intermediate form is as close to SPARQL as possible, while still retaining generalizability. 
%     % @Srini 1. Need to provide evidence for KG transfer (say increased Hits@1) on one QA dataset after training embeddings on another QA dataset. Relations must overlap for this. Evidence-Train embeddings on lcquad2.0, test on SimpleQuestions-wiki. @Srini 2. Prove assertion of QA having greater inductive bias because of closed-world assumption. Evidence-In MetaQA, train using closed and open world assumption, check which is higher.
%     % \item The method and motivation for fine-tuning KG embeddings using multi-hop QA data. The derivation of \textit{relation composition} functions for some popular link prediction scoring functions, to do the above. If possible, show embeddings-based KG interaction \textit{also} transfers across multiple datasets for the same KG.
%     \item Architecture that separates the semantic parsing and KG interaction steps; such that Semantic parsing transfers across datasets. involves: A simple seq2seq baseline that explicitly recognizes the decomposed relations of the question using KB vocabulary (eg. the SPARQL), and then chooses the top predicted query that exists in the KG. 
%     % does standard link prediction using the above fine-tuned embeddings to obtain the answer.
 
% \end{enumerate}


==> sections/kbqa.tex <==
%\section{Knowledge Base Question Answering}
\subsection{Task Definition}
% Let $\mathcal{E} = \{e_0 ...e_N\}$ be a set of entities, and $\mathcal{R} = \{r_0 ...r_M\}$ be a set of relations. 
% A knowledge fact is a triple $<e_s, r, e_o>$ that describes the relationship between a subject and an object entity. 
% A knowledge graph $\mathcal{G}$ is defined by the tuple $\big(\mathcal{E}, \mathcal{R}, \mathcal{F}\big)$, where $\mathcal{F} = \{<e_s, r, e_o>\} \subseteq \mathcal{E}\times\mathcal{R}\times\mathcal{E}$ is the set of fact triples.

% The input to the \kbqa task is a natural language question $q$ to be answered based on the facts available in the knowledge graph $\mathcal{G}$. 
% % In this work, we consider the settings in which a structured query $S$ is available at training, given that $S$ best represents the expected behavior of $q$ over the knowledge graph $\mathcal{G}$ to produce the answer $a$. 

% % \begin{equation}
% %     Pr(a \mid q, \mathcal{G}) = \sup_{S} Pr(a, S \mid q, \mathcal{G})
% % \end{equation}

% % There are two types of structured query $S$ that are commonly used for \kbqa. The \textit{logical form queries} \citep{pasupat2016inferring, guo2018dialog, shen2019multi} express reasoning steps toward the answer using a pre-defined $\lambda$-calculus grammar.
% % The \sparql \textit{queries} join together all of the triples with a matching subject, relation or object, then apply some \textsc{Sql}-like operations such as \textsc{Ask} or \textsc{Select}. 
% We consider \sparql query as the intermediate structured query $S$. 
% We assume optimal \sparql queries are given from expert annotators, and these queries always execute to target answers.
% Then, our goal is to estimate the likelihood of generating the structured query given the question and the knowledge graph.

% \begin{equation}
%     Pr(a \mid q, \mathcal{G}) = Pr(S \mid q, \mathcal{G})
% \end{equation}



%Formally defining the semantic parsing based methodology to KBQA, given a natural language question $\mathbf{Q}$, and a knowledge graph $\mathbf{K = E R E}$ where $\mathbf{E}$ are entities in the $\mathbf{K}$ and $R$ are edge labels that are relationships connecting two entities, the goal is to transform $Q$ to a SPARQL query $S = C \bigcup Q_g$ 


The KBQA task involves finding an answer in a given Knowledge Graph $\mathcal{G} ; <V, E>$ for a natural question $q$. We consider the setting where a structured query exists that can retrieve the correct answer(s) is present in the KG, and we solve the task by learning a distribution over \sparql{}s to find the correct structured query that would retrieve the required answers, i.e, $$Pr(\sparql | q, G)$$



 
